Describing Nuclear Matter with Effective Field Theories

An accurate description of nuclear matter starting from free-space nuclear forces has been an elusive goal. The complexity of the system makes approximations inevitable, so the challenge is to find a consistent truncation scheme with controlled errors. The virtues of an effective field theory approach to this problem are discussed.

==> jimdefs.tex <==
%auto-ignore
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\ben}{\begin{eqnarray*}}
\newcommand{\een}{\end{eqnarray*}}

\def\simlt{\stackrel{<}{{}_\sim}}
\def\simgt{\stackrel{>}{{}_\sim}}
\newcommand{\lnablasq}{\overleftarrow{\nabla}{}^{\!2}}
\newcommand{\rnablasq}{\overrightarrow{\nabla}{}^{\!2}}
\newcommand{\wt}{\widetilde}
\def\({\left( }
\def\){\right) }
\def\[{\left[ }
\def\]{\right] }

\newcommand{\Real}{\mbox{Re}\,}
\newcommand{\Imag}{\mbox{Im}\,}
\newcommand{\order}{{\cal O}}

%EFT Defs
\newcommand{\drms}{DR[$\overline{\mbox{MS}}$]}
\newcommand{\Mbar}{\frac{M}{4\pi}(\mu+ip)}
\newcommand{\sing}{$^1\!S_0$ }
\newcommand{\trip}{$^3\!S_1$ }
\newcommand{\psing}{$^1\!P_1$ }
\newcommand{\LambdaNN}{\Lambda_{{\rm NN}}}

